q2d: Turning Questions into Dialogs to Teach Models How to Search

One of the exciting capabilities of recent language models for dialog is their ability to independently search for relevant information to ground a given dialog response. However, obtaining training data to teach models how to issue search queries is time and resource consuming. In this work, we propose q2d: an automatic data generation pipeline that generates information-seeking dialogs from questions. We prompt a large language model (PaLM) to create conversational versions of question answering datasets, and use it to improve query generation models that communicate with external search APIs to ground dialog responses. Unlike previous approaches which relied on human written dialogs with search queries, our method allows to automatically generate query-based grounded dialogs with better control and scale. Our experiments demonstrate that: (1) For query generation on the QReCC dataset, models trained on our synthetically-generated data achieve 90%--97% of the performance of models trained on the human-generated data; (2) We can successfully generate data for training dialog models in new domains without any existing dialog data as demonstrated on the multi-hop MuSiQue and Bamboogle QA datasets. (3) We perform a thorough analysis of the generated dialogs showing that humans find them of high quality and struggle to distinguish them from human-written dialogs.

==> figs_and_tables/table_ablation_filters.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{\begin{tabular}{@{}ccc@{}}
\toprule
Threshold & \% Mean Score & \% Rouge-1 Recall \\ \midrule
0         & 72          & 68              \\
0.25      & 78          & 70                \\
0.5       & 83          & 71                \\
0.75      & 91          & 75                \\
0.8       & 93          & 76                \\
0.9       & 97          & 77                \\
0.95      & 99          & 79                \\
0.99      & 100         & 81                \\ \bottomrule
\end{tabular}}
\caption{Evaluation set performance increases as reverse filtering thresholds are raised.}
\label{tab:ablation_filters}
\end{table}

==> figs_and_tables/table_results_extending.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
\toprule
                 & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}SBERT \\ Similarity\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Rouge-1\\ Recall\end{tabular}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Search Results\\ Recall@10\end{tabular}} \\ \midrule
Model / Test Set & M                                      & B                                      & M                                     & B                                    & M                                          & B                                         \\ \midrule
WizInt           & 66                                     & 67                                     & 40                                    & 36                                   & 21                                         & 21                                        \\
BlenderBot3      & 62                                     & 69                                     & 32                                    & 35                                   & 19                                         & 24                                        \\
LaMDA            & 72                                     & 75                                     & 63                                    & 63                                   & 31                                         & 34                                        \\
T5 (QReCC)       & 74                                     & 77                                     & 70                                    & 65                                   & 34                                         & 37                                        \\
PaLM 540B        & 88                                     & 82                                     & 81                                    & 69                                   & 52                                         & 41                                        \\
Flan-U-PaLM 540B & 89                                     & 82                                     & 83                                    & 68                                   & 57                                         & 39                                        \\ \midrule
\textbf{LaMDA (MuSiQue)}  & 98                                     & 90                                     & 93                                    & 76                                  & 72                                         & 50                                         \\
\textbf{T5 (MuSiQue)}     & 97                                     & 91                                     & 94                                    & 80                                   & 75                                         & 54                                        \\ \bottomrule
\end{tabular}
}
\caption{Language and dialogue models results on query generation test sets. The M/B numbers indicates results on MuSiQue auto-generated dialogues / Bamboogle manually constructed dialogues. (QReCC) / (MuSiQue) indicates additional fine-tuned on a q2d dataset. The models that achieved the best results are the models fine-tuned on the auto-generated MuSiQue dialogue. After fine-tuning on MuSiQue auto-generated, LaMDA and T5 results improve by 20\%-70\% on the human annotated test. The improvement also correlates with improvements on the auto-generated test set -- showing our method effectiveness also for creating evaluation data.}
\label{tab:results_extending}
\end{table}

==> figs_and_tables/table_results_replacing.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllll@{}}
\toprule
Model                  & Training Dataset & \begin{tabular}[c]{@{}c@{}}SBERT \\ Similarity\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Rouge-1\\ Recall\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Search Results\\ Recall@10\end{tabular}  \\ \midrule
\multirow{2}{*}{T5}    & Human Annotated                   & 92.4                                                          & 88.1                                                       & 68.5                                                                 \\
                       & Auto Generated                    &
                       87.5 (\textbf{95\%})                                                          & 83.3 (\textbf{95\%})                                                       & 61.5 (\textbf{90\%})                                                                 \\ \midrule
\multirow{3}{*}{LaMDA} & None                              & 81.2                                                          & 77.8                                                       & 48.4                                                                 \\
                       & Human Annotated                   & 92.1                                                          & 87.5                                                       & 67.9                                                                 \\
                       & Auto Generated                    &  89.4 (\textbf{97\%})                                                           &   84.8 (\textbf{97\%})                                                       &    63.3 (\textbf{93\%})                                                                \\ \bottomrule
\end{tabular}}
\caption{Results on the human-annotated QReCC NQ test set, experimenting with replacing the human-annotated data with automatically generated data with the \emph{q2d} method. Bold shows the percentage of performance for a model trained with auto-generated data out of a model trained with human-annotated data. Training on the automatically generated data achieves 90\%-97\% of the model trained on the human annotated results.}
\label{tab:results_replaing}
\end{table}

==> sections/98_background.tex <==
Large language models (LLMs) and dialog models like LaMDA  \cite{thoppilan2022lamda} and BlenderBot \cite{shuster2022blenderbot} need to be grounded in factual information from the real world \cite{shuster2022language}. For example, if a model is trained in 2019 and asked ``How old is Joe Biden?'', we expect it to provide a factual response even in 2023. \enav{another aspect the factuality path solves is that of hallucinations. We should emphasis that freshness and hallucinations avoidance are two separate issues addressed by this path.} Human conversations often contain questions about previously discussed topics, sometimes using anaphora. For instance, a conversation may start by discussing an entity (e.g., ``Joe Biden'') and later ask a related question (e.g., ``How old is he anyway?''). In order to provide reliable and consistent answers, it is necessary to generate a decontextualized query (e.g., "How old is Joe Biden") for a search engine \cite{parisi2022talm,kasai2022realtime,press2022measuring}.  \enav{this pragrpah sounds more like an intro paragraph to me than a background paragraph. I would expect examples to appear in the intro, and this section to be more concrete, citing relevant work.}

Using APIs also allows for decoupling language and reasoning from knowledge \cite{borgeaud2021improving,parisi2022talm}. Models store information in their parameters, which can cause errors when the data becomes outdated. As an example, if a model is trained in 2020 and asked "How old is the current president?", it may produce the incorrect query "How old is Donald Trump" due to outdated parameters or hallucinations. We deal with the use-case of multi-hop QA in Section~\ref{sec:extending}.

% \enav{I wouldn't say they use it in several ways , but rather that they use it through the following pipeline of models}
LaMDA and BlenderBot use the search API to communicate in several ways: (a) Research triggering: A classifier that determines whether the current turn requires communicating with the search API. (b) Query generation: Given the current dialog, generate a concrete, decontextualized (no anaphora and all relevant entities included) search query. (c) Response generation: Obtain search results, generate candidate responses, and select the best one. Our work focuses on the query generation component and shows how improving the query leads to more factual responses.
